Guessing Smart: Biased Sampling for Efficient Black-Box Adversarial Attacks

We consider adversarial examples for image classification in the black-box decision-based setting. Here, an attacker cannot access confidence scores, but only the final label. Most attacks for this scenario are either unreliable or inefficient. Focusing on the latter, we show that a specific class of attacks, Boundary Attacks, can be reinterpreted as a biased sampling framework that gains efficiency from domain knowledge. We identify three such biases, image frequency, regional masks and surrogate gradients, and evaluate their performance against an ImageNet classifier. We show that the combination of these biases outperforms the state of the art by a wide margin. We also showcase an efficient way to attack the Google Cloud Vision API, where we craft convincing perturbations with just a few hundred queries. Finally, the methods we propose have also been found to work very well against strong defenses: Our targeted attack won second place in the NeurIPS 2018 Adversarial Vision Challenge.

==> 7_playground.tex <==
\section{Playground}
\[
\Pr_{S\sim D^m} [L_D(h)>\epsilon] < \delta
\]

\[
\Pr_{S\sim D^m} [L_D(h)>\min_{h'\in H}L_D(h') +\epsilon] < \delta
\]

\[
m\geq m^{UC}(\epsilon, \delta)
\]

\[
m\geq m_H^{NUL}(\epsilon, \delta, h)
n
\]


\[
d(s_{pred},s_{valid}) \approx 0.057
d(s_{invalid},s_{valid}) \approx 0.667
\]

\[
\vec{s}_{valid}  \vec{s}_{invalid} \vec{s}_{uncertain}
\]


==> 9999_challenge.tex <==
\section{Evaluation} 	\label{sec:eval}	

We evaluate our approach in three steps: First, we present a range of experiments and our winning submission to the NeurIPS 2018 Adversarial Vision Challenge. Next, we attack an ImageNet classifier and compare our results to other proposed Black-box attacks. Finally, we mount an attack against the Google Cloud Vision API and show that our method is efficient 
against real-world commercial systems.

\subsection{Adversarial Vision Challenge}

When evaluating adversarial attacks and defenses, it is hard to obtain meaningful results. Very often, attacks are tested against weak defenses and vice versa, and results are cherry-picked. We sidestep this problem by instead submitting our approach to the  Adversarial Vision Challenge (AVC), where our method is pitted against state-of-the-art robust models and black-box defenses. 

\textbf{Evaluation setting}. The AVC is an open competition between image classifiers and adversarial attacks in an iterative black-box decision-based setting \cite{avc2018}. Participants can choose between three tracks:
\begin{itemize}
	\item Robust model: The submitted code is a robust image classifier. The goal is to maximize the $\ell^2$ norm of any successful adversarial perturbation.
	\item Untargeted attack: The submitted code must find a perturbation that changes classifier output, while minimizing the $\ell^2$ distance to the original image.
	\item Targeted attack: Same as above, but the classification must be changed to a specific label.
\end{itemize}

Attacks are continuously evaluated against the current top-5 robust models and vice versa. Each evaluation run consists of 200 images with a resolution of 64x64, and the attacker is allowed to query the model 1000 times for each image. The final attack score is then determined by the median $\ell^2$ norm of the perturbation over all 200 images and top-5 models (lower is better).

At the time of writing, the exact methods of most model submissions were not yet published. But seeing as more than 60 teams competed in the challenge, it is reasonable to assume that the top-5 models accurately depict the state of the art in adversarial robustness. We know through personal correspondence that most winning models used variations of Ensemble Adversarial Training \cite{tramer17ens}, while denoisers were notably absent from at least the top 3.

\textbf{Dataset}. The models are trained with the Tiny ImageNet dataset, which is a down-scaled version of the ImageNet classification dataset, limited to 200 classes with 500 images each. Model input consists of color images with 64x64 pixels, and the output is one of 200 labels. The evaluation is conducted with a secret hold-out set of images, which is not contained in the original dataset and unknown to participants of the challenge. 


\subsubsection{Random guessing with low frequency}

Before implementing the Biased Boundary Attack, we first conduct a simple experiment to demonstrate the effectiveness of Perlin noise patterns against strong defenses. Specifically, we run a random-guessing attack that samples candidates uniformly from the surface of a $\ell^2$-hypersphere with radius $\epsilon$ around the original image:
$$s \sim \mathcal{N}(0, 1)^k;\ x_{adv} = x_0 + \epsilon \cdot \frac{s}{\|s\|_2}$$

With a total budget of 1000 queries to the model for each image, we use binary search to reduce the sampling distance $\epsilon$ whenever an adversarial example is found. First experiments have indicated that the targeted setting may be too difficult for pure random guessing. Therefore we limit this experiment to the untargeted attack track, where the probability of randomly sampling \textit{any  of 199} adversarial labels is reasonably high.

We add a second attack, replacing the distribution with normalized Perlin noise:

$$s \sim Perlin_{64,64}(v);\ x_{adv} = x_0 + \epsilon \cdot \frac{s}{\|s\|_2}$$

We set the Perlin frequency to 5 for all attacks on Tiny ImageNet. Figure \ref{fig:figure-perlin} shows adversarial examples from both distributions. As Table \ref{tab1} shows, Perlin patterns are more efficient and the attack finds adversarial perturbations with much lower distance (63\% reduction), supporting the findings independently made by Guo et al. \cite{guo2018low}. Although intended as a dummy submission to the AVC, this attack was already strong enough for a top-10 placement in the untargeted track.




\begin{table}[htbp]
	\caption{Random guessing with low frequency (untargeted).}
	\label{tab1}
	\vskip 0.1in
	\begin{center}
		\begin{small}
			\begin{sc}
				\begin{tabular}{lr}
					%\toprule
					Distribution & Median $\ell^2$ distance \\
				\hline
					Normal 			& 11.15 \\
					\textbf{Perlin noise (ours)}	& \textbf{4.28} \\
					%\bottomrule
				\end{tabular}
			\end{sc}
		\end{small}
	\end{center}
	\vskip -0.1in
\end{table}



\subsubsection{Biased Boundary Attack}

\begin{figure}[htb]
	\centering
	(a) \includegraphics[width=.215\textwidth]{img/sala-1-img.png} \ \ 
	\includegraphics[width=.215\textwidth]{img/sala-1-diff.png} 
	\\
	\ 
	\\
	
	(b) \includegraphics[width=.215\textwidth]{img/sala-2-img.png} \ \ 
	\includegraphics[width=.215\textwidth]{img/sala-2-diff.png} 
	\\
	\ 
	\\
	
	(c) \includegraphics[width=.215\textwidth]{img/sala-3-img.png} \ \ 
	\includegraphics[width=.215\textwidth]{img/sala-3-diff.png} 
	
	\caption{Comparision of Boundary Attack and Biased Boundary Attack after 1000 queries. While originally a "european fire salamander", all three images are classified as "sulphur butterfly". (a) Boundary Attack: $d_{\ell^2} = 9.4$ (b) BBA with Perlin bias: $d_{\ell^2} = 7.5$ (c) BBA with Perlin and projected gradient biases: $d_{\ell^2} = 4.4$. See Appendix \ref{appendix_tiny} for more examples.}
	\label{fig:salamander-bba}	
\end{figure}



Next, we evaluate the Biased Boundary Attack in our intended setting, the targeted attack track in the AVC. 

To provide a point of reference, we first implement the original Boundary Attack, and initialize it with known images from the target class. Specifically, we use the training set of Tiny ImageNet, and from all images of the target class we pick the one with the lowest distance to the source image. The Boundary Attack works, but is too slow for our setting. Compare Figure \ref{fig:salamander-bba}a, where the starting point (a butterfly) is still clearly visible after 1000 iterations.
%The Boundary attack then interpolates towards the decision boundary, and along it towards the original.




We then implement the Biased Boundary Attack by adding our first prior, low-frequency noise (see Figure \ref{fig:salamander-bba}b). As before, we simply replace the distribution from which the attack samples the orthogonal step with Perlin patterns. As shown in Table \ref{tab2}, this alone decreases the median $\ell^2$ distance by 25\%.  

Finally, we add projected gradients from a surrogate model and set the bias strength $w$ to 0.5. This further reduces the median $\ell^2$ distance by another 37\%, or a total of 53\% when compared with the original Boundary Attack. 1000 iterations are enough to make the butterfly almost invisible to the human eye (Figure \ref{fig:salamander-bba}c). See Appendix \ref{appendix_tiny} for more adversarial examples generated on Tiny ImageNet.


\begin{table}[htp]
	\caption{Biases for the Boundary Attack (targeted).}
	\label{tab2}
	\vskip 0.15in
	\begin{center}
		\begin{small}
			\begin{sc}
				\begin{tabular}{lcr}
					%\toprule
					Attack & Bias & Median $\ell^2$  \\
					\hline
					Boundary Attack	& - 			& 20.2 \\
					BBA (ours)		& Perlin		& 15.1 \\
					\textbf{BBA (ours)}		& \textbf{Perlin + PG}	& \textbf{9.5} \\
					%\bottomrule
				\end{tabular}
			\end{sc}
		\end{small}
	\end{center}
	%\vskip -0.1in
\end{table}


In our submission to the AVC, we used an ensemble of ResNet18 and ResNet50, both of which are public baselines provided by the competition organizers. This ensemble is reasonably strong, but not state-of-the-art (the ResNet50 baseline was trained with Adversarial Logit Pairing, which has since been shown to be less effective than originally assumed \cite{alp1, alp2}). In fact, most winning submissions to the AVC used much larger ensembles of carefully-trained models\footnote{ See blog post at \footnotesize \url{https://medium.com/bethgelab/}}. This reinforces the claim that our method outperforms most existing attacks even when using simple surrogate models.


\subsection{Comparison on ImageNet}
\label{sec:eval-imagenet}

The AVC has shown that our attack is very efficient against strong defenses. However, we note that the dataset (Tiny ImageNet) is not in widespread use. To compare our method to established black-box attacks, we therefore implement it for an ImageNet classifier. 

\textbf{Setting}. ImageNet consists of images with 299x299 color pixels, and has 1000 classes. We use a pre-trained InceptionV3 network \cite{inceptionv3}, which achieves 78\% top-1 accuracy. It does not employ any defenses against adversarial examples - our attack is therefore evaluated in the most common setting. 

\textbf{Other methods}. We compare the Biased Boundary Attack to the Boundary Attack, both in its original \cite{brendel17} and low-frequency form \cite{guo2018low}. We also include approaches proposed by Ilyas et al. \cite{ilyas18a} and Cheng et al. \cite{chengHardlabel}. As an additional point of reference, we include the score-based methods ZOO \cite{zoo} and AutoZOOM \cite{autozoom}. 

\textbf{Evaluation}. Our attack always starts with an image of the adversarial class, therefore success must be characterized by low distance to the source image. For this, we define thresholds on the $\ell^2$-norm of the adversarial perturbation, and register success when the distance is below. We create an evaluation set by randomly drawing 1000 images from the ImageNet validation set, run each attack on this set and report the average \textit{success rate} over all images. 

For the gradient bias in the BBA, we use the adversarially trained Inception-Resnet-v2 model of Tram{\`e}r et al. \cite{tramer17ens} and set the bias strength $w$ to 0.5. We do not perform any training ourselves. For the low-frequency bias, we set the Perlin frequency to 20.

\subsubsection{Untargeted ImageNet attack}

Arguably, untargeted attacks on ImageNet do not accurately represent a real-world scenario. After all, changing a "persian cat" to a "egyptian cat" is hardly malicious for most use cases. Nevertheless, we include this experiment since some methods \cite{guo2018low,chengHardlabel} report only untargeted results on ImageNet. We run all attacks for 4000 queries and fix the success threshold to a MSE of 0.001 ($d_{\ell^2}$ = 16.38), which is the setting used by Guo et al. 

\begin{table*}[htp]
	\caption{Untargeted attack on ImageNet. \textit{Results marked with (*) are reported by the respective authors, and not evaluated by us.}}
	\label{tab_imagnet_untarg}
	\vskip 0.1in
	\begin{center}
		\begin{small}
			\begin{sc}
				\begin{tabular}{lccccccr}
%					\toprule
					\ & \multicolumn{6}{c}{Success rate vs number of queries}  \\
					\  & 250 & 500 & 1000 & 2000 & 4000 & 150\hspace{.15em}000+   \\
					\hline
					Boundary Attack & 0.38 & 0.46 & 0.49 & 0.52	& 0.53 & \textbf{1.00} (*) \\
					Cheng et al. \cite{chengHardlabel} & 0.24 & 0.37 & 0.37 & 0.39 & 0.39 & \textbf{1.00} (*) \\
					Guo et al. \cite{guo2018low} & 0.41 & 0.45 & 0.53 & 0.64 & 0.70 & - \\
					BBA (Perlin, Ours) & 0.39 & 0.47 & 0.61 & 0.62 & 0.69 & -	\\
					BBA (Perlin + PG, Ours) & \textbf{0.44} & \textbf{0.62} & \textbf{0.72} & \textbf{0.75} & \textbf{0.76} & -	\\
%					\bottomrule
				\end{tabular}
			\end{sc}
		\end{small}
	\end{center}
	%\vskip -0.1in
\end{table*}

\textbf{Discussion}. Table \ref{tab_imagnet_untarg} shows that our attack is successful after very few iterations, and is the most efficient by far for low query counts. It is also apparent that our low-frequency patterns are similar in performance to those of Guo et al. \cite{guo2018low}. As an aside, our experiment sees them start with much higher success rate (41\% after 250 iterations versus 9\% reported by them). This is due to our choice of initialization method: Instead of adding Gaussian noise to the source image, we search the ImageNet validation set and pick the closest image to the source. 


\subsubsection{Targeted ImageNet attack} 
\label{sec_eval_imagenet_targ}

\todo{First, show bias comparison.}

\todo{We go on to benchmark our method against a range of state-of-the-art attacks. In all cases, we use the code provided by the respective authors. We do not change any hyperparameters, but modify the implementations to run on our evaluation set and to using the same target classes and starting points. In this way, all attacks are benchmarked on the exact same images.}

We repeat the same experiment in a targeted setting over 15000 queries and fix a random target label for each example in the evaluation set (all attacks run on the same image/target combinations). Since some of the methods we compare \cite{ilyas18a} use $\ell^\infty$ distance exclusively, we set the $\ell^2$-threshold to 25.89. This corresponds to a worst-case $\ell^\infty$-distortion of 0.05 if one assumes all pixels to be maximally perturbed. Appendix \todo{Ref appendix} shows selected examples of this evaluation.

\begin{figure}[htb]
	\centering
	\includegraphics[width=.45\textwidth]{img/imagenet.png} \ \ 

	
	\caption{Query-distortion study of the targeted Biased Boundary Attack on ImageNet.}
	\label{fig:imagenet-graph}	
\end{figure}

\textbf{Discussion}. As Figure \ref{fig:imagenet-graph} shows, our attack is very efficient below 10000 queries, but later slows down drastically. In Table \ref{tab_imagnet_targ}, we see that there exist methods with higher success rates, but they need significantly more queries to achieve them. Unfortunately, the authors do not report results at low query counts.

The only attacks that are comparable in efficiency are score-based gradient estimators. This is of little value to our setting, but it  still confirms that these methods should be used whenever scores are available. Nevertheless, our evaluation shows that the BBA is the most efficient attack in a label-only few-query scenario.


\begin{table*}[htp]
	\caption{Targeted attack on ImageNet. The BBA is the most efficient attack in a label-only setting. However, score-based estimators still perform better if scores are indeed available. \textit{Results marked with (*) are reported by the respective authors, and not evaluated by us.}}
	\label{tab_imagnet_targ}
	\vskip 0.1in
	\begin{center}
		\begin{small}
			\begin{sc}
				\begin{tabular}{lcccccccr}
					\ & \multicolumn{7}{c}{Success rate vs number of queries} & Median queries \\
					\  & 500 & 1000 & 2500 & 5000 & 10000 & 15000 & 1M+ & until success \\
					\hline
					\textit{Label-only} & & & & & & & & \\
					Ilyas et al. \cite{ilyas18a} (label-only) & - & - & - & - & - & - & \textbf{0.9} (*) & 2.7M (*) \\
					Boundary Attack & 0.01 & 0.02 & 0.06 & 0.12	& 0.23 & 0.31 & - & 6263 \\
					BBA (Perlin, Ours) & 0.01 & 0.03 & \textbf{0.15} & 0.24 & 0.32 & 0.40 & - & 5541	\\
					BBA (Perlin + PG, Ours) & \textbf{0.05} & \textbf{0.08} & 0.14 & \textbf{0.27} & \textbf{0.50} & \textbf{0.63} & - & \textbf{3406}	\\
					
					\hline
					\textit{Using confidence scores}  & & & & & & & & \\
					ZOO \cite{zoo} & - & - & - & - & - & - & 0.76 (*) & 2.2M (*)	\\
					AutoZOOM \cite{autozoom} & - & - & - & - & - & \textbf{0.99} (*) & - & 13525 (*)	\\
					Ilyas et al. \cite{ilyas18a} (General) & - & - & - & - & - & 0.98 (*) & - & \textbf{11550} (*) \\

				\end{tabular}
			\end{sc}
		\end{small}
	\end{center}
	%\vskip -0.1in
\end{table*}

\begin{table*}[htp]
	\caption{Comparison }
	\label{tab_targ_bias_comp}
	\vskip 0.1in
	\begin{center}
		\begin{small}
			\begin{sc}
				\begin{tabular}{ccc|rrrrrr|c}
					\multicolumn{3}{c|}{Active biases} & \multicolumn{6}{c|}{Success rate vs number of queries} & Median queries \\
					Perlin & Mask & gradient  & 500 & 1000 & 2500 & 5000 & 10000 & 15000 & until success \\
					\hline

					no &no&no& 0.01 & 0.02 & 0.06 & 0.12	& 0.23 & 0.31 & 6263 \\
					yes &no&no& 0.01 & 0.03 & \textbf{0.15} & 0.24 & 0.32 & 0.40 & 5541	\\
					no & yes &no& 0.01 & 0.02 & 0.06 & 0.12	& 0.23 & 0.31 & 6263 \\					
					yes & yes &no& 0.01 & 0.02 & 0.06 & 0.12	& 0.23 & 0.31 & 6263 \\
					no &no& yes & 0.01 & 0.02 & 0.06 & 0.12	& 0.23 & 0.31 & 6263 \\					
					yes &no& yes & \textbf{0.05} & \textbf{0.08} & 0.14 & \textbf{0.27} & \textbf{0.50} & \textbf{0.63} & \textbf{3406}	\\
					no & yes & yes & 0.01 & 0.02 & 0.06 & 0.12	& 0.23 & 0.31 & 6263 \\
					yes & yes & yes & 0.01 & 0.02 & 0.06 & 0.12	& 0.23 & 0.31 & 6263 \\

				\end{tabular}
			\end{sc}
		\end{small}
	\end{center}
	%\vskip -0.1in
\end{table*}


\subsection{Google Cloud Vision API}
\label{google_attack}

To show that our method can be efficient even against commercial black box classifiers, we conduct an attack against the Google Cloud Vision API. This is significantly harder than attacking ImageNet, since the exact classes are unknown. In order to craft adversarial examples in less than 1000 queries, we relax the attack formulation:

\textbf{Multi-targeted attack}. We have argued earlier that untargeted attacks with many redundant classes are not truly adversarial. However, the opposite is also true: to achieve an adversarial effect, it is not always necessary to target one specific class. Rather, the same effect could be achieved by targeting a group of classes - if we want to label a dog as a cat, we can take the union of all cat breeds to achieve the desired effect. This greatly simplifies the task and allows us to conduct a targeted attack against the Google Cloud Vision API with high success chance.

\textbf{Turning a person into a bear.} To conduct an attack with this goal, we relax the target ("bear") and formulate the adversarial criterion as:
\begin{itemize}
	\item One of the top-3 labels must contain the word "bear" (this includes grizzly bear, brown bear, etc.)
	\item The words "face", "facial expression", "skin", "person" must not appear in any of the output labels.
\end{itemize}

\begin{figure}[htb]
	\centering
	\includegraphics[width=.45\textwidth]{img/google2.png} \ 
	\caption{Clean image classified by Google Cloud Vision.}
	\label{fig:googleclean}	
\end{figure}

\begin{figure}[htb]
	\centering
	\includegraphics[width=.45\textwidth]{img/google1.png} \ 
	\caption{Adversarial image (target "bear") classified by Google Cloud Vision after 346 queries. There are no other labels, i.e. Google Cloud Vision outputs only three results. See Appendix \ref{appendix_google} for more examples.}
	\label{fig:googleadv}	
\end{figure}

We use the exact same implementation that we submitted to the AVC, since it is already heavily optimized. Unfortunately, this limits us to a resolution of 64x64 (see Appendix \ref{appendix_google} for an experiment at ImageNet resolution). 

Figures \ref{fig:googleclean} and \ref{fig:googleadv} show the result: after only 346 iterations, our attack produces a perturbation that is still visible ($d_{\ell^2}=5.86$), but small enough to fool an unsuspecting person. This demonstrates once more the key strength of our attack: instead of aiming for perfect adversarial examples, we achieve sufficiently good results with a very low number of queries. Again, it should be stressed that we do \textit{not} use confidence scores (even though they are available here).


\ \\
\ \\




==> 9_references.tex <==
% NOTE: This is not IEEE Style, which definitely sucks.

\begin{thebibliography}{00}
\bibitem{b1} Szegedy, C., Zaremba, W., Sutskever, I., Bruna, J., Erhan, D., Goodfellow, I., \& Fergus, R. (2014). Intriguing properties of neural networks. In \textit{International Conference on Learning Representations}. Retrieved from \url{https://arxiv.org/abs/1312.6199}

\bibitem{b2} Goodfellow, I., Shlens, J., \& Szegedy, C. (2015). Explaining and Harnessing Adversarial Examples. In \textit{International Conference on Learning Representations}. Retrieved from \url{https://arxiv.org/abs/1412.6572}

\bibitem{b3} Carlini, N., \& Wagner, D. (2017). Towards Evaluating the Robustness of Neural Networks. In \textit{IEEE Symposium on Security and Privacy}, 39-57. Retrieved from \url{https://arxiv.org/abs/1608.04644}

\bibitem{b4} Madry, A., Makelov, A., Schmidt, L., Tsipras, D., \& Vladu, A. (2018). Towards deep learning models resistant to adversarial attacks. In \textit{International Conference on Learning Representations}. Retrieved from \url{https://arxiv.org/abs/1706.06083}

\bibitem{b5} Ilyas, A., Engstrom, L., Athalye, A., \& Lin, J. (2018). Black-box Adversarial Attacks with Limited Queries and Information. In \textit{International Conference on Machine Learning}. Retrieved from \url{https://arxiv.org/abs/1804.08598}

\bibitem{b6} Brendel, W., Rauber, J., \& Bethge, M. (2018). Decision-based adversarial attacks: Reliable attacks against black-box machine learning models. In \textit{International Conference on Learning Representations}. Retrieved from \url{https://arxiv.org/abs/1712.04248}

\bibitem{b7} Tram\`{e}r, F., Papernot, N., Goodfellow, I., Boneh, D., \& McDaniel, P. (2017). The space of transferable adversarial examples. \textit{arXiv preprint}. Retrieved from  \url{https://arxiv.org/abs/1704.03453}

\bibitem{b8} Tram\`{e}r, F., Kurakin, A., Papernot, N., Goodfellow, I., Boneh, D., \& McDaniel, P. (2018). Ensemble adversarial training: Attacks and defenses. In \textit{International Conference on Learning Representations}. Retrieved from  \url{https://arxiv.org/abs/1705.07204}

\bibitem{b9} Athalye, A., Carlini, N., \& Wagner, D. (2018). Obfuscated gradients give a false sense of security: Circumventing defenses to adversarial examples. In \textit{International Conference on Machine Learning}. Retrieved from \url{https://arxiv.org/abs/1802.00420}

\bibitem{b10} Kurakin, A., Goodfellow, I., Bengio, S., Dong, Y., Liao, F., Liang, M., ... \& Wang, J. (2018). Adversarial attacks and defences competition. \textit{arXiv preprint}. Retrieved from  \url{https://arxiv.org/abs/1804.00097}

\bibitem{b11} Liao, F., Liang, M., Dong, Y., Pang, T., Zhu, J., \& Hu, X. (2017). Defense against adversarial attacks using high-level representation guided denoiser. \textit{arXiv preprint}. Retrieved from \url{https://arxiv.org/abs/1712.02976}

\bibitem{b12} Xie, C., Wang, J., Zhang, Z., Ren, Z., \& Yuille, A. (2018). Mitigating adversarial effects through randomization. In \textit{International Conference on Learning Representations}. Retrieved from \url{https://arxiv.org/abs/1711.01991}

\bibitem{b13} Athalye, A., Engstrom, L., Ilyas, A. \& Kwok, K. (2018). Synthesizing robust adversarial examples. In \textit{International Conference on Machine Learning}. Retrieved from \url{https://arxiv.org/abs/1707.07397}

\bibitem{b14} Perlin, K. (1985). An image synthesizer. In \textit{ACM Siggraph Computer Graphics}, 19(3), 287-296.

\bibitem{b15} Guo, C., Frank, J., \& Weinberger, K. (2018). Low Frequency Adversarial Perturbation. \textit{arXiv preprint}. Retrieved from \url{https://arxiv.org/abs/1809.08758}

\bibitem{b16} Brendel, W., Rauber, J., Kurakin, A., Papernot, N., Veliqi, B., Salathé, M., ... \& Bethge, M. (2018). Adversarial vision challenge. \textit{arXiv preprint}. Retrieved from \url{https://arxiv.org/abs/1808.01976}

\bibitem{b17} Engstrom, L., Ilyas, A., \& Athalye, A. (2018). Evaluating and understanding the robustness of adversarial logit pairing. In \textit{Neural Information Processing Systems}. Retrieved from \url{https://arxiv.org/abs/1807.10272}

\bibitem{b18} Mosbach, M., Andriushchenko, M., Trost, T., Hein, M., \& Klakow, D. (2018). Logit Pairing Methods Can Fool Gradient-Based Attacks. In \textit{Neural Information Processing Systems}. Retrieved from \url{https://arxiv.org/abs/1810.12042}

\bibitem{b19} Brendel, W. (2018). Results of the NIPS Adversarial Vision Challenge 2018. Retrieved from \url{https://medium.com/bethgelab/results-of-the-nips-adversarial-vision-challenge-2018-e1e21b690149}

\end{thebibliography}

